SLaM: Student-Label Mixing for Distillation with Unlabeled Examples

Knowledge distillation with unlabeled examples is a powerful training paradigm for generating compact and lightweight student models in applications where the amount of labeled data is limited but one has access to a large pool of unlabeled data. In this setting, a large teacher model generates ``soft'' pseudo-labels for the unlabeled dataset which are then used for training the student model. Despite its success in a wide variety of applications, a shortcoming of this approach is that the teacher's pseudo-labels are often noisy, leading to impaired student performance. In this paper, we present a principled method for knowledge distillation with unlabeled examples that we call Student-Label Mixing (SLaM) and we show that it consistently improves over prior approaches by evaluating it on several standard benchmarks. Finally, we show that SLaM comes with theoretical guarantees; along the way we give an algorithm improving the best-known sample complexity for learning halfspaces with margin under random classification noise, and provide the first convergence analysis for so-called ``forward loss-adjustment" methods.

==> tables/celeba-hard-comparison-table.tex <==

\begin{table*}[t] 
\renewcommand{\arraystretch}{1.15}
\caption{Experiments on CelebA (\textbf{hard}-distillation). See Section~\ref{comparison_with_previous} for details.}
\label{tab:celeba-hard-comparison}
\begin{center}
\tiny
\begin{tabular}{|c| c c c c c c|} 
 \hline
Labeled Examples  & $2\%$ & $3\%$ & $4\%$ & $5\%$ & $6\%$  & $7\%$\\  
 \hline
 Teacher  & 
 $86.19$ & 
 $88.25$ & 
 $88.95$ & 
 $91.31$ & 
 $92.09$ & 
 $92.62$\\ 
\hline
 Vanilla & 
   $89.73  \pm 0.08$ &
   $91.61  \pm 0.09$ &
   $92.05  \pm 0.11$ &
   $93.41  \pm 0.13$ &
   $94.02  \pm 0.15$ &
   $94.05  \pm 0.04$\\
 \hline
 % PolyLoss \cite{leng2022polyloss}  & 
 %   $89.73  \pm 0.12$ &
 %   $91.65  \pm 0.03$ &
 %   $92.21  \pm 0.21$ &
 %   $93.51  \pm 0.07$ &
 %   $94.03  \pm 0.11$ &
 %   $94.15  \pm 0.10$\\
 Taylor-CE \cite{feng2021can} &   
 $ \mathbf{90.62 \pm 0.05}$ & 
 $ 92.19\pm  0.02$ & 
 $ 92.66\pm  0.11 $ &
 $ 93.60 \pm 0.14$ & 
 $ 94.00 \pm 0.04$ & 
 $ 94.38 \pm 0.10$ \\
 \hline
 UPS \cite{rizvedefense} &   
 $ 89.35 \pm 0.04 $ & 
 $ 91.30 \pm 0.04$ & 
 $ 91.95 \pm 0.12$ &
 $ 93.18 \pm 0.07$ & 
 $ 93.71 \pm 0.04$ & 
 $ 94.18 \pm 0.03$ \\
 \hline
 VID \cite{Ahn2019CVPR} & 
 % $\mathbf{90.88 \pm 0.21}$ &           
 % $\mathbf{92.74 \pm 0.09}$ &           
 % $\mathbf{93.33 \pm 0.11}$ &           
 % $\mathbf{94.01\pm 0.10}$ &
 % $\mathbf{94.65 \pm 0.15}$ &
 % $\mathbf{94.77 \pm 0.13} $
$ 89.92 \pm 0.21 $ &
$91.60 \pm  0.11$ &
$92.20 \pm  0.12$ &
$93.51 \pm 0.15$ &
$94.08 \pm 0.15 $ &
$94.27 \pm 0.10$
 \\
 \hline
 Weighted \cite{IKBMTV22} &
$90.06 \pm 0.06 $ &
$91.97\pm 0.13 $ &
$92.45\pm 0.10 $ &
$93.60\pm 0.07 $ &
$93.94\pm 0.12  $ &
$94.25\pm 0.16  $\\

 \hline
 SLaM (Ours) & 
 $90.43 \pm 0.05$ &
 $\mathbf{92.25 \pm 0.11}$ &
 $\mathbf{92.71 \pm 0.08}$ &
 $\mathbf{93.96 \pm 0.17}$ &
 $\mathbf{94.39 \pm 0.21}$ &
 $\mathbf{94.52 \pm 0.12}$ \\
 \hline
\end{tabular}

\end{center}

\end{table*}



==> tables/celeba-soft-comparison-table.tex <==


\begin{table*}[t] 
\renewcommand{\arraystretch}{1.15}
\caption{Experiments on CelebA (\textbf{soft}-distillation). See Section~\ref{comparison_with_previous} for details.}
\label{tab:celeba-soft-comparison}
\begin{center}
\tiny
\begin{tabular}{|c| c c c c c c|} 
 \hline
Labeled Examples  & $2\%$ & $3\%$ & $4\%$ & $5\%$ & $6\%$  & $7\%$\\  
 \hline
 Teacher  & 
 $86.19$ & 
 $88.25$ & 
 $88.95$ & 
 $91.31$ & 
 $92.09$ & 
 $92.62$\\ 
\hline
 Vanilla & 
 $89.96 \pm 0.08$ &
 $91.55 \pm 0.14$ &
 $92.16 \pm 0.10$ &
 $93.42 \pm 0.06$ &
 $93.98 \pm 0.04$ &
$94.29 \pm 0.03$\\
 \hline
 Taylor-CE \cite{feng2021can} &   
 $\mathbf{90.80 \pm 0.07}$ & 
 $ \mathbf{92.23 \pm 0.1} $ & 
 $ 92.56 \pm 0.14$ &
 $ 93.80 \pm 0.20$ & 
 $ 94.17 \pm 0.07$ & 
 $ 94.47 \pm 0.01$ \\
 \hline
 UPS \cite{rizvedefense} &   
 $89.96 \pm 0.11 $ & 
 $92.03 \pm 0.09$ & 
 $92.44 \pm 0.04$ &
 $93.9 \pm 0.05$ & 
 $94.28 \pm 0.07$ & 
 $94.68 \pm 0.03$ \\
%  \hline
%  PolyLoss \cite{leng2022polyloss} &   
%   $89.96 \pm 0.10$ &
%  $91.61 \pm 0.05$ &
%  $92.17 \pm 0.09$ &
%  $93.57 \pm 0.17$ &
%  $94.01  \pm 0.11$ &
% $94.32 \pm 0.08$\\
 \hline
 VID \cite{Ahn2019CVPR} & 
  $89.91 \pm 0.10$ &
  $91.75 \pm 0.21$ &
  $92.21 \pm 0.10$ &
  $93.67 \pm 0.21$ &       
  $94.15 \pm 0.07 $ &
  $94.33 \pm 0.16 $ \\
 \hline
 
 Weighted \cite{IKBMTV22} &  
  $89.92 \pm 0.12$ &
  $91.73 \pm 0.09$ &
  $92.31 \pm 0.22$ &
  $93.64 \pm 0.10$ &
  $93.93 \pm 0.14$ &
  $94.23 \pm 0.11$  \\
 \hline
 SLaM (Ours) &  
  $90.37 \pm 0.17$ &
  $\mathbf{92.25 \pm 0.11}$ &
  $\mathbf{92.74 \pm 0.17}$ &
  $\mathbf{94.06 \pm 0.07}$ &
  $\mathbf{94.39 \pm 0.10}$ &
  $ \mathbf{94.75 \pm 0.08}$\\
 \hline
\end{tabular}

\end{center}


\end{table*}



==> tables/cifar10-hard-comparison-table.tex <==
\begin{table*}[t] 
\renewcommand{\arraystretch}{1.15}
\caption{Experiments on CIFAR-10 (\textbf{hard}-distillation). See Section~\ref{comparison_with_previous} for details.}
\label{tab:cifar10-hard-comparison}
\begin{center}
\tiny
\begin{tabular}{|c| c c c c c c|} 
 \hline
Labeled Examples  & $5000$ & $7500$ & $10000$ & $12500$ & $15000$  & $17500$\\  
 \hline
 Teacher  & $61.30 $ & $68.98 $ & $72.42 $ & $73.92 $ & $ 76.63 $  & $78.63 $\\ 
\hline
 Vanilla & 
$ 62.26 \pm 0.45$ &
$ 69.07 \pm 0.11$ &
$ 72.09 \pm 0.11$ &
$ 73.43 \pm 0.16$ &
$ 75.93 \pm 0.25$ &
$ 77.43\pm  0.15$\\
 \hline
 % PolyLoss \cite{leng2022polyloss}  & 
 %  $61.84 \pm 0.45$ &
 %  $69.03 \pm 0.09$ &
 %  $71.86 \pm 0.07$ & 
 %  $74.20 \pm 0.30$ & 
 %  $76.41 \pm 0.18$ & 
 %  $77.66 \pm 0.11$\\
 %   \hline
 Taylor-CE \cite{feng2021can} &   
 $ 63.14 \pm 0.07$ & 
 $ 69.98 \pm 0.11$ & 
 $ 72.72 \pm 0.36 $ &
 $ 73.77 \pm 0.28 $ & 
 $ 76.26 \pm 0.29 $ & 
 $ 77.88 \pm 0.20 $ \\
 \hline
 UPS \cite{rizvedefense} &   
 $  64.27 \pm 0.08$ & 
 $  70.93 \pm 0.26 $ & 
 $  73.78 \pm 0.16$ &
 $  74.66\pm  0.29$ & 
 $  77.38 \pm 0.37$ & 
 $  78.95\pm  0.08$ \\
 \hline
 VID \cite{Ahn2019CVPR} & 
 $ 61.95 \pm 0.22 $ &           
 $ 66.91 \pm 0.21$ &           
 $ 69.59 \pm 0.24$ &           
 $ 72.16 \pm 0.47 $ &
 $ 74.83 \pm 0.11 $ &
 $ 75.55 \pm 0.21 $ \\
 \hline
 Weighted \cite{IKBMTV22} &
$63.22 \pm 0.45 $ &
$71.04 \pm 0.26 $ &
$72.84 \pm 0.12$ &
$74.20 \pm 0.16$ &
$76.56 \pm 0.24$ &
$78.23 \pm 0.15$\\

 \hline
 SLaM (Ours) & 
 $\mathbf{66.40 \pm 0.31}$ &
 $\mathbf{72.44 \pm 0.17}$ &
 $\mathbf{74.77 \pm 0.13}$ &
 $\mathbf{75.64 \pm 0.19}$ &
 $\mathbf{77.99 \pm 0.36}$ & 
 $\mathbf{79.26 \pm 0.26}$ \\ 
 \hline
\end{tabular}

\end{center}

\end{table*}


==> tables/cifar10-soft-comparison-table.tex <==

% \begin{table*}[t] 
% \renewcommand{\arraystretch}{1.15}
% \caption{Experiments on CIFAR-10 (\textbf{soft}-distillation). See Section~\ref{comparison_with_previous} for details.}
% \label{tab:cifar10-soft-comparison}

% \begin{center}
% \tiny
% \begin{tabular}{|c| c c c c c c|} 
%  \hline
% Labeled Examples  & $5000$ & $7500$ & $10000$ & $12500$ & $15000$  & $17500$\\  
%  \hline
%  Teacher  & $61.78 $ & $68.43 $ & $72.42 $ & $74.73 $ & $ 77.31 $  & $78.86 $\\ 
% \hline
%  Vanilla & 
%  $62.60 \pm 0.40$ &  
%  $69.88 \pm 0.06$ & 
%  $72.71 \pm 0.20 $ & 
%  $75.21 \pm 0.15 $ & 
%  $77.32 \pm 0.12 $ & 
%  $78.68 \pm 0.16$ \\
%  \hline
%  PolyLoss \cite{leng2022polyloss} &   
%  $63.02 \pm 0.23$ & 
%  $69.89 \pm 0.17$ & 
%  $73.12 \pm 0.11$ &
%  $75.33 \pm 0.21$ & 
%  $77.64 \pm 0.31$ & 
%  $78.92 \pm 0.23$ \\
 
%  \hline
%  Taylor-CE \cite{feng2021can} &   
%  $63.02 \pm 0.23$ & 
%  $69.89 \pm 0.17$ & 
%  $73.12 \pm 0.11$ &
%  $75.33 \pm 0.21$ & 
%  $77.64 \pm 0.31$ & 
%  $78.92 \pm 0.23$ \\
 
%  \hline
%  UPS \cite{rizvedefense} &   
%  $63.02 \pm 0.23$ & 
%  $69.89 \pm 0.17$ & 
%  $73.12 \pm 0.11$ &
%  $75.33 \pm 0.21$ & 
%  $77.64 \pm 0.31$ & 
%  $78.92 \pm 0.23$ \\
%  \hline
 
%  VID \cite{Ahn2019CVPR} & 
%  $63.26 \pm 0.13$ & 
%  $70.01 \pm 0.30$ & 
%  $73.07 \pm 0.21$ & 
%  $75.22 \pm 0.28$ & 
%  $77.62 \pm 0.05$ & 
%  $78.52 \pm 0.21$ \\  
%  \hline
%  Weighted \cite{IKBMTV22} &  
%  $63.42 \pm 0.21$ & 
%  $70.73 \pm 0.40$ & 
%  $73.54 \pm 0.12$ & 
%  $75.92 \pm 0.30$ & 
%  $77.71 \pm 0.24$ & 
%  $79.01 \pm 0.30 $\\
%  \hline
%  SLaM (Ours) &  
%  $\mathbf{65.78 \pm 0.10}$ & 
%  $\mathbf{72.07 \pm 0.34}$ & 
%  $\mathbf{74.57 \pm 0.17}$ & 
%  $\mathbf{76.88 \pm 0.12}$ & 
%  $\mathbf{78.51 \pm 0.14}$ & 
%  $\mathbf{79.47 \pm 0.15}$ \\
%  \hline
% \end{tabular}
% \end{center}


% \end{table*}

\begin{table*}[t] 
\renewcommand{\arraystretch}{1.15}
\caption{Experiments on CIFAR-10 (\textbf{soft}-distillation). See Section~\ref{comparison_with_previous} for details.}
\label{tab:cifar10-soft-comparison}

\begin{center}
\tiny
\begin{tabular}{|c| c c c c c c|} 
 \hline
Labeled Examples  & $5000$ & $7500$ & $10000$ & $12500$ & $15000$  & $17500$\\  
 \hline
 Teacher  & $61.30 $ & $68.98 $ & $72.42 $ & $73.92$ & $ 76.63 $  & $78.63$\\ 
\hline
 Vanilla & 
 $ 63.53 \pm 0.29$ &  
 $70.39 \pm 0.11 $ & 
 $ 73.23 \pm 0.15 $ & 
 $74.29 \pm 0.25 $ & 
 $ 76.64 \pm 0.20 $ & 
 $ 78.63 \pm 0.16$ \\
 % \hline
 
 % PolyLoss \cite{leng2022polyloss} &   
 % $66.19 \pm 0.14$ & 
 % $72.40 \pm 0.12$ & 
 % $73.51 \pm 0.43$ &
 % $75.84 \pm 0.23$ & 
 % $78.07 \pm 0.05$ & 
 % $79.21 \pm 0.41$ \\
 
 \hline
 Taylor-CE \cite{feng2021can} &   
 $64.07 \pm 0.26$ & 
 $71.19 \pm 0.17$ & 
 $74.18 \pm 0.25$ &
 $74.65 \pm 0.24$ & 
 $77.17 \pm 0.04$ & 
 $78.67 \pm 0.13$ \\
 
 \hline
 UPS \cite{rizvedefense} &   
 $ 64.56 \pm 0.13$ & 
 $ 71.10 \pm 0.34$ & 
 $ 74.17 \pm 0.06$ &
 $ 75.05 \pm 0.24$ & 
 $ 77.64 \pm 0.12$ & 
 $ \mathbf{79.21 \pm 0.27} $ \\
 \hline
 
 VID \cite{Ahn2019CVPR} & 
 $63.76 \pm 0.13$ & 
 $70.58 \pm 0.17$ & 
 $73.77 \pm 0.40$ & 
 $74.95 \pm 0.21$ & 
 $77.25 \pm 0.06$ & 
 $78.23 \pm 0.09$ \\  
 \hline
 
 Weighted \cite{IKBMTV22} &  
 $63.85 \pm 0.13$ & 
 $71.04 \pm 0.24$ & 
 $73.64 \pm 0.36$ & 
 $75.00 \pm 0.17$ & 
 $77.40 \pm 0.17$ & 
 $78.93 \pm 0.19$ \\
 \hline
 
 SLaM (Ours) &  
 $\mathbf{66.82 \pm 0.61}$ & 
 $\mathbf{72.61 \pm 0.30}$ & 
 $\mathbf{75.01 \pm 0.25}$ & 
 $\mathbf{75.72 \pm 0.17}$ & 
 $\mathbf{78.04 \pm 0.16}$ & 
 $\mathbf{79.22 \pm 0.11}$ \\
 \hline
\end{tabular}
\end{center}


\end{table*}

==> tables/cifar100-hard-comparison-table.tex <==

\begin{table*}[t] 
\renewcommand{\arraystretch}{1.15}
\caption{Experiments on CIFAR-100 (\textbf{hard}-distillation). See Section~\ref{comparison_with_previous} for details.}
\label{tab:cifar100-hard-comparison}
\begin{center}
\tiny
\begin{tabular}{|c| c c c c c c|} 
 \hline
Labeled Examples  & $5000$ & $7500$ & $10000$ & $12500$ & $15000$  & $17500$\\  
 \hline
 Teacher  & 35.97 & 44.65 & 49.62 & 55.68 & 59.19 & 62.05 \\
\hline
 Vanilla &  
 $36.36 \pm 0.04$ & 
 $44.15 \pm 0.10$ & 
 $50.22 \pm 0.07$ & 
 $55.55 \pm 0.24$ & 
 $58.85 \pm 0.1$  & 
 $61.43 \pm 0.19$\\
 \hline
 % PolyLoss \cite{leng2022polyloss}  &  
 % $36.78 \pm 0.16$ &
 % $44.58 \pm 0.30$ &
 % $50.23 \pm 0.19$ &
 % $55.40 \pm 0.34$ &
 % $59.10 \pm 0.31$ &
 % $61.57 \pm 0.28$\\
 % \hline
  Taylor-CE \cite{feng2021can} &   
 $ 39.12 \pm 0.14$ & 
 $ 46.87 \pm 0.10$ & 
 $ 52.64 \pm 0.22$ &
 $ 57.19 \pm 0.28$ & 
 $ 59.95 \pm 0.11$ & 
 $ 62.36 \pm 0.21$ \\
 \hline
 UPS \cite{rizvedefense} &   
 $ 39.49\pm 0.13$ & 
 $ 48.36\pm 0.44$ & 
 $ 53.95\pm 0.10$ &
 $ 57.95\pm 0.10$ & 
 $ 60.59\pm 0.29$ & 
 $ 62.09\pm 0.28$ \\
 \hline
 VID \cite{Ahn2019CVPR} & 
 $37.19 \pm 0.09$ &
 $44.67 \pm 0.16$ &
 $50.63 \pm 0.35$ &
 $54.78 \pm 0.07$ &
 $59.27 \pm 0.14$ &
 $62.01 \pm 0.05$\\
 \hline
 Weighted \cite{IKBMTV22} & 
 $38.04 \pm 0.29$ & 
 $46.45 \pm 0.22$ & 
 $52.33 \pm 0.18$ & 
 $57.43 \pm 0.13$ & 
 $60.81 \pm 0.09$ & 
 $63.02 \pm 0.06$\\
 \hline
 SLaM (Ours) & 
 $\mathbf{42.01 \pm 0.29}$ & 
 $\mathbf{49.08 \pm 0.14}$ & 
 $\mathbf{54.49 \pm 0.17}$ & 
 $\mathbf{58.53 \pm 0.04}$ &
 $\mathbf{61.12 \pm 0.15}$ & 
 $\mathbf{63.21 \pm 0.18}$\\
 \hline
\end{tabular}

\end{center}


\end{table*}



==> tables/cifar100-soft-comparison-table.tex <==

\begin{table*}[t] 
\renewcommand{\arraystretch}{1.15}
\caption{Experiments on CIFAR-100 (\textbf{soft}-distillation). See Section~\ref{comparison_with_previous} for details.}
\label{tab:cifar100-soft-comparison}
\begin{center}
\tiny
\begin{tabular}{|c| c c c c c c|} 
 \hline
Labeled Examples  & $5000$ & $7500$ & $10000$ & $12500$ & $15000$  & $17500$\\  
 \hline
 Teacher  & $35.97$ & $44.65$ & $49.62$ & $55.68$ & $59.19$ & $62.05$ \\
\hline
 Vanilla & 
 $37.94 \pm 0.10$ & 
 $46.42 \pm 0.24$ & 
 $52.17 \pm 0.21$ & 
 $57.72 \pm 0.17$ & 
 $60.91 \pm 0.07$ & 
 $63.47 \pm0.23$\\
 % \hline
 % PolyLoss \cite{leng2022polyloss} & 
 % $38.01 \pm 0.18$ &  
 % $46.64 \pm 0.31$ & 
 % $52.23 \pm 0.22$ & 
 % $57.95 \pm 0.13$ & 
 % $61.07 \pm 0.09$ & 
 % $63.67 \pm 0.02$\\
 \hline
 Taylor-CE \cite{feng2021can} &   
 $40.18 \pm 0.07$ & 
 $48.05 \pm 0.29$ & 
 $54.08 \pm 0.24$ &
 $58.45 \pm 0.17$ & 
 $61.13 \pm 0.10$ & 
 $63.54 \pm 0.26 $ \\
 
 \hline
 UPS \cite{rizvedefense} &   
 $39.62 \pm 0.23$ & 
 $48.48 \pm 0.15$ & 
 $54.43\pm 0.27$ &
 $58.17 \pm 0.07$ & 
 $60.74 \pm 0.10$ & 
 $62.13 \pm 0.12$ \\
 \hline
 VID \cite{Ahn2019CVPR} &  
  $38.93 \pm 0.39$ &
  $46.76 \pm 0.10$ &
  $52.56 \pm 0.17$ &
  $57.94 \pm 0.37$ &
  $61.14 \pm 0.28$ &
  $63.56 \pm 0.18$\\  
 \hline
 Weighted \cite{IKBMTV22} &  
 $38.63 \pm 0.32$ & 
 $47.11 \pm 0.29$ & 
 $53.16 \pm 0.25$ & 
 $58.20 \pm 0.11$ & 
 $\mathbf{61.29 \pm 0.15}$ & 
 $63.58 \pm 0.07$\\
 \hline
 SLaM (Ours) & 
 $\mathbf{42.72 \pm 0.30}$ & 
 $\mathbf{49.89 \pm 0.23}$ & 
 $\mathbf{54.73 \pm 0.27}$ & 
 $\mathbf{58.78 \pm 0.15}$ & 
 $\mathbf{61.30 \pm 0.09}$ & 
 $\mathbf{63.98 \pm 0.19}$\\
 \hline
\end{tabular}

\end{center}

\end{table*}


==> tables/cifar100-temperature.tex <==
\begin{table*}[t] 
\renewcommand{\arraystretch}{1.15}
\caption{CIFAR-100 Temperature Ablation. See \Cref{app:sec:temperature-composability} for a plot of the results.}
\label{CIFAR100_temperature}
\begin{center}
\tiny
\begin{tabular}{|c| c c c c c c|} 
 \hline
Labeled Examples  & $10\%$ & $15\%$ & $20\%$ & $25\%$ & $30\%$  & $35\%$\\  
 \hline
 Teacher  & 35.97 & 44.65 & 49.62 & 55.68 & 59.19 & 62.05 \\
\hline
 Vanilla + Temperature &  
 $42.24 \pm 0.21$ & 
 $49.43 \pm 0.17$ & 
 $53.97 \pm 0.08$ & 
 $57.85 \pm 0.15$ & 
 $61.32 \pm 0.13$ & 
 $63.55 \pm 0.10$\\
 \hline
 SLaM (Ours) + Temperature & 
 $\mathbf{43.43 \pm 0.29}$ & 
 $\mathbf{50.84 \pm 0.14}$ & 
 $\mathbf{54.68 \pm 0.09}$ & 
 $\mathbf{59.12 \pm 0.10}$ &
 $\mathbf{61.38 \pm 0.15}$ & 
 $\mathbf{64.00 \pm 0.18}$\\
 \hline
\end{tabular}

\end{center}

\end{table*}

==> tables/imagenet-soft-comparison-table.tex <==

\begin{table*}[t!] 
\renewcommand{\arraystretch}{1.15}
\caption{Experiments on ImageNet (\textbf{soft}-distillation). See Section~\ref{comparison_with_previous} for details.}
\label{tab:imagenet-soft-comparison}
\begin{center}
\tiny
\begin{tabular}{|c| c c c c c c|} 
 \hline
Labeled Examples  & $5\%$ & $10\%$ & $15\%$ & $20\%$ & $25\%$ & $30\%$ 
\\  
 \hline
 Teacher  & $39.48$ & $52.96 $ & $59.64 $ & $63.62$ & $66.00$ & $67.85$\\ 
 \hline
 Vanilla & 
 $41.67 \pm 0.05$ & 
 $55.9 \pm 0.06$ & 
 $62.3 \pm 0.09$ & 
 $65.91 \pm 0.05$ &
 $67.98 \pm 0.07$ &
 $69.12 \pm 0.08$ 
 \\
 \hline
  Taylor-CE \cite{feng2021can} &   
  $41.61 \pm 0.06	$ &
  $56.43 \pm 0.06	$ &
  $62.38 \pm 0.11	$ &
  $65.86 \pm 0.08	$ &
  $67.70 \pm 0.22	$ &
  $68.62 \pm 0.07$ \\
 % PolyLoss \cite{leng2022polyloss} & 
 % $43.89 \pm 0.1$ &  
 % $58.06 \pm 0.07$ & 
 % $63.97 \pm 0.1$ & 
 % $\mathbf{67.12 \pm 0.04}$ \\
 \hline
 VID \cite{Ahn2019CVPR} &  
  $40.12 \pm 0.04$ &
  $52.75 \pm 0.04$ &
  $58.01 \pm 0.03$ &
  $61.21 \pm 0.06$ &
  $62.37 \pm 0.06$ &
  $63.05 \pm 0.07$
  \\  
 \hline
 Weighted \cite{IKBMTV22} &  
 $41.67 \pm 0.04$ & 
 $55.96 \pm 0.07$ & 
 $62.29 \pm 0.08$ & 
 $65.91 \pm 0.05$ &
 $ 67.96 \pm 0.06$ &
 $\mathbf{69.16 \pm 0.08} $ 
 \\
 \hline
 SLaM (Ours) & 
 $\mathbf{48.1 \pm 0.05}$ & 
 $\mathbf{59.51 \pm 0.07}$ & 
 $\mathbf{64.08 \pm 0.06}$ & 
 $ \mathbf{66.72 \pm 0.11}$  &
 $ \mathbf{68.17 \pm 0.07} $ &
 $ 69.07 \pm 0.05 $
 \\
 \hline
\end{tabular}

\end{center}

\end{table*}


==> tables/imdb-soft-comparison-table.tex <==
\begin{table*}[t] 
\renewcommand{\arraystretch}{1.15}
\caption{Experiments on the Large Movies Reviews Dataset (\textbf{soft}-distillation). See Section~\ref{app:imdb-comparison} for details.}
\label{tab:imdb-soft-comparison}

\begin{center}
\tiny
\begin{tabular}{|c| c c c c |} 
 \hline
Labeled Examples  & $2\%$ & $4\%$ & $8\%$ & $40\%$ 
% & $10\%$ & $16\%$
\\  
 \hline
 Teacher  & $77.52$	& $84.04$	& $85.44$	& $88.3$\\
\hline
 Vanilla & 
 $80.93 \pm 0.10$ & 
 $85.12 \pm 0.29$ & 
 $85.99 \pm 0.08$ & 
 $87.50 \pm 0.6$  \\
 \hline
%  PolyLoss \cite{leng2022polyloss} & 
% $81.26 \pm 0.08$ &
% $85.19 \pm 0.14$ &
% $85.96 \pm 0.19$ &
%  $87.58 \pm 0.46$\\
%  \hline
  Taylor-CE \cite{feng2021can} &   
 $ 79.5 \pm 0.38 $ & 
 $ 85.14 \pm 0.13$ & 
 $ 85.98 \pm 0.14$ &
 $ 87.57\pm 0.3$ \\
 \hline
 VID \cite{Ahn2019CVPR} &  

$ 81.76 \pm 0.32$ &
$85.33 \pm 0.35 $ &
$86.17 \pm 0.06 $ & 
$87.71 \pm 0.01 $ 
\\  
 \hline
 Weighted \cite{IKBMTV22} &  
$ 81.1 \pm +0.1 $&
$85.2 \pm 0.05$  &
$86.13 \pm 0.17 $&	
$\mathbf{87.8 \pm 0.25}$  \\
 \hline
 SLaM (Ours) & 

$ \mathbf{81.88 \pm 0.23}$	&
$ \mathbf{85.5 \pm 0.09}$ &
$ \mathbf{86.23 \pm 0.13}$ &
$87.73 \pm 0.38$  \\
 \hline
\end{tabular}

\end{center}

\end{table*}






